Recovering Variable Names for Minified Code with Usage Contexts

In modern Web technology, JavaScript (JS) code plays an important role. To avoid the exposure of original source code, the variable names in JS code deployed in the wild are often replaced by short, meaningless names, thus making the code extremely difficult to manually understand and analysis. This paper presents JSNeat, an information retrieval (IR)-based approach to recover the variable names in minified JS code. JSNeat follows a data-driven approach to recover names by searching for them in a large corpus of open-source JS code. We use three types of contexts to match a variable in given minified code against the corpus including the context of properties and roles of the variable, the context of that variable and relations with other variables under recovery, and the context of the task of the function to which the variable contributes. We performed several empirical experiments to evaluate JSNeat on the dataset of more than 322K JS files with 1M functions, and 3.5M variables with 176K unique variable names. We found that JSNeat achieves a high accuracy of 69.1%, which is the relative improvements of 66.1% and 43% over two state-of-the-art approaches JSNice and JSNaughty, respectively. The time to recover for a file or for a variable with JSNeat is twice as fast as with JSNice and 4x as fast as with JNaughty, respectively.

==> combination.tex <==
\section{Usage context combination}
When recovering a name for a varible, single-variable, multiple-variable usage context and task-specific context should be taken into account together because each of them affects the variable. Therefore, we introduce an approach using combination between the contexts to recover the minified variable names. There are 4 type of combinations as subsections belows.
\subsection{Task + SingleVar}
Given a minified function named \texttt{fn} in which variable \texttt{v} is used, the probability of variable name \texttt{vn} could be named to \texttt{v} is computed as the following formula:
\begin{equation}
PTS_{v, vn} = \alpha * VFAS_{vn, fn} + \beta * SGCS_{v, vn}
\end{equation}
%
where, $VFAS_{vn, fn}$ is vairable-function association score between \texttt{vn} and \texttt{fn}, $SGCS_{v, vn}$ is StarGraph confident score of variable name \texttt{vn} with \texttt{vn}, $\alpha$ and $\beta$ are weighted parameters. 

\subsection{Task + MultiVar}
\subsection{SingleVar + Multiple Var}
\subsection{Task + SingleVar + Multiple Var}

==> context_matchin_singleVar.tex <==
%\subsection{Context matching for given minified code}

%A variable in a function has a certain context which is represented
%by its relation graph. Generally, if 2 variables have the same
%context, they often are named similarly.  Therefore, to determine a
%name for a variable, we can seek in the corpus as if there exist
%another variable which has the similar context with the mininied
%variable.  Given a minified code which has \texttt{n} variables,
%recovering name for these variables is finding variables in the
%corpus whose relation graphs match with these variables' relation
%graph.  Corpus is a set of variables' relation graphs which are mined
%from a large training data mentioned in section \texttt{VII}.

%\newtheorem*{graph_matching}{Graph matching}
%\begin{graph_matching}
%A relation graph $sg_0$ is considered to be matched with relation graph $sg_1$ if only if $\varphi$ percentage of number edges in $sg_1$ could be found in $sg_0$.
%\end{graph_matching}

%In reality, it is very difficult to find 2 graphs matching completely
%because there are a variety of usage for each variable and their
%relation graphs could be built from a huge number of different
%edges. Therefore, $\varphi$ is used as a threshold to determine
%whethere 2 graphs are matched.


==> dbBuild.tex <==
%From a JS file
% Parse
%		What is local/global
%		StarGraph
% StarGraph
\label{sectionDbBuild}
For a JavaScript file, we parse and built its Abstract Syntax Tree (AST) with Mozilla Rhino. The file is discarded if it cannot be parsed. From the AST of the code,
% we identify global and local variables by: If a variable is declared, but is not wrapped in any function, it is considered as a global one. If a variable is declared or passed as argument inside a function, it is considered as a local one. Since global variables are not minified by obfuscating tools like UglifyJS \cite{}, we simply count the number of global variables as base line 
we proceed to build the relation graph data and the association data as follows:
\subsubsection{Relation graph data}
We make a relation graph for each local variable of a scope with the center of the graph as the variable itself. Then, we determine the variable's properties and role relations with other non-variables program entities. A variable's properties are found by traversing all the function call and field access AST nodes in which the variable is the receiver. A variable's role relations are found by traversing all the binary expression AST nodes that have the variable as one of its child node; the remaining child node is related to the variable through the parent node. If that child node is not a leaf node, we use the right most leaf node of its subtree as the label for the role relation. Each property/role is built into the relation graph as a node marked with its name and an edge connected to the center node which describes the property/relation. For the example in figure \ref{example_sim}, the relation graph for the \texttt{dataTransfer} has 6 nodes: the center node (the variable itself), a node \texttt{getData()} with edge named function call, a node \texttt{types} with edge named field access, a node \texttt{clipboardData} with edge named assignment, a node \texttt{dataTransfer} with edge named assignment, and a node \texttt{getData} with edge named field access. Overall, each JavaScript file has a set of distinctive relationship graphs represent its local variables.
\\
\subsubsection{Association data}
To collect the frequency of variable names which usually go together, first, for each function, we determine all of its local variables. Then based on the configuration of our algorithm, we would extract pairs or triplets of variable names that appear together in the function, and increment the count of that pair/triplets in the corpus. 


==> main.tex <==
\section{Single-variable usage context}
%TODO HIEU
\section{Multiple-variable usage context}
%TODO HIEU
\section{Task-specific context}
%TODO HIEU

\section{Combination of contexts for name recovery}
%TODO HIEU

\section{{\tool}: Approach...}
\subsection{Database Building}
%TODO NGOC

\subsection{Name recovery algorithm}
%TODO HIEU

\section{}


==> multiVar_ConfidentScore.tex <==
% Algorithm - Calculate confident score

%\textit{Confiden Score.} 

The score (MC) for a set of $n$ recovered names in a partially recovered
result (will be explained in \textbf{S.3}) for $n$ variables represents the likelihood of co-occurrences
of these names in a function. It is computed:
\begin{equation}
\label{confidentScore}
MC_{vn_1, vn_2, ..., vn_n} = \frac{\sum_{j=1}^{n_{subJ}} assoc(S_j)}{n_{subJ}}
\end{equation}

Assume that we have a set of $n$ variable names, and the name of $i^{th}$
variable is $vn_i$. Due to the fact that not all possible sets of $n$
names appear together in a corpus, we compute the score based on the
associations of all subsets of the size $J$ with $J$ <=~$n$.
%
$S_j$ is a subset of size $J$ of $(vn_1, vn_2, ..., vn_n)$; $n_{subJ}$
is the number of such subset; and $assoc(S_j)$ is the association
score of all variable names in set $s_j$ (computed by
Formula~\ref{eq:assocN}).

%$assoc(x^j_1, x^j_2, ... , x^j_n)$ is the association score for the
%set $s_j$, and $x^j_1, x^j_2, ... , x^j_n$ is variable names in set
%$s_j$.


%Confident score of a set of $n$ variable names is the score which presents the probability of co-occurence of these $n$ variable names in a function. The confident score of a set expresses how likelihood these names appearing together. Therefore, we use association score for confident score calculation.






%The confident score of this set is computed as the formula \ref{confidentScore} below.
%\begin{equation}
%\label{confidentScore}
%CF_{vn_1, vn_2, ..., vn_n} = \frac{\sum_{j=1}^{n_{subJ}} assoc(s_j)}{n_{subJ}}
%\end{equation}
%
%\begin{equation}
%\label{assocSet}
%assocSet(s_j) = assoc(x^j_1, x^j_2, ... , x^j_n)
%\end{equation}

%where, $s_j$ is a subset of size $J$ of $(vn_1, vn_2, ..., vn_n)$,
%$n_{subJ}$ is the number of such subset,
%$assoc(s_j)$ is the association score of all variable names in set $s_j$, which could be computed in formula \ref{eq:assocN}
%$assoc(x^j_1, x^j_2, ... , x^j_n)$ is the association score for the set $s_j$, and $x^j_1, x^j_2, ... , x^j_n$ is variable names in set $s_j$.

